FETA: A Benchmark for Few-Sample Task Transfer in Open-Domain Dialogue

Task transfer, transferring knowledge contained in related tasks, holds the promise of reducing the quantity of labeled data required to fine-tune language models. Dialogue understanding encompasses many diverse tasks, yet task transfer has not been thoroughly studied in conversational AI. This work explores conversational task transfer by introducing FETA: a benchmark for few-sample task transfer in open-domain dialogue. FETA contains two underlying sets of conversations upon which there are 10 and 7 tasks annotated, enabling the study of intra-dataset task transfer; task transfer without domain adaptation. We utilize three popular language models and three learning algorithms to analyze the transferability between 132 source-target task pairs and create a baseline for future work. We run experiments in the single- and multi-source settings and report valuable findings, e.g., most performance trends are model-specific, and span extraction and multiple-choice tasks benefit the most from task transfer. In addition to task transfer, FETA can be a valuable resource for future research into the efficiency and generalizability of pre-training datasets and model architectures, as well as for learning settings such as continual and multitask learning.

==> sections/analysis.tex <==
\section{Results and Analysis}
\label{sec:analysis}

\subsection{Single-Source Setting}
Table \ref{tab:overall_transfer} shows the average and top-1 scores and $\Delta$s for all three models and algorithms and we use this table to understand general trends. Figure \ref{fig:main_heatmaps} shows the relative improvement of a source task for each target task, demonstrating trends across tasks.

\begin{figure*}
    \centering
    \includegraphics[width=\textwidth]{images/transfer_heatmaps.png}
    \caption{\textbf{Relative improvement of transfer over baselines}. Rows are source tasks and columns are target tasks. Diagonal cells are baseline scores. Looking at an individual column can demonstrate best source tasks for that target, while looking at rows can determine which source task works well across multiple targets. Note that DailyDialog (left) and Friends (right) have different scales. \textcolor{blue}{Is a task name mapping necessary?}}
    
    %Task abbreviations are as follows: ER - emotion recognition, DAC - dialog act classification, TC - topic classification, CESE - causal emotion span extraction, CEE - causal emotion entailment, DNLI - dialogue-level NLI, DRSE - dialogue reasoning span extraction, DRMC - dialogue reasoning multiple choice, CRE - commonsense relation extraction, ARS - adversarial response selection, EER - emotion recognition (EmoryNLP), RC - reading comprehension, CI - character identification, QA - question answering, PD - personality detection, RE - relation extraction, MER - emotion recognition (MELD).\textcolor{blue}{Is this mapping necessary?}
    \label{fig:main_heatmaps}
\end{figure*}

\paragraph{Aggregate Task Transfer Performance}
 First, we find that the Friends tasks get scores that are between 7-8 points lower than the DailyDialog tasks on average. This is likely due to the increased number of speakers and utterance length in the Friends dataset, making it more challenging. The highest average score across both is just over 50\%, demonstrating that there is significant room for improvement on the tasks in both datasets. Additionally, the highest average $\Delta$ is only 1.4, demonstrating that there is still significant room for improvement in transfer algorithms. Furthermore, we find the mean difference between average $\Delta$ and top-1 $\Delta$ to be over 1.6, suggesting that there is significant benefit to understanding which tasks transfer best.

\paragraph{Performance Across Models} When considering raw scores, BERT and T5 are competitive with each other on both DailyDialog and Friends, but GPT-2's performance lags behind by ~10 points. This is not unexpected as autoregressive decoder models are not designed with classification tasks in mind. Interestingly, when considering score $\Delta$s, the ranking of model performance differs depending on the dataset. On DailyDialog, T5 gets the best performance increase by using task transfer, followed by GPT-2 and BERT. However, we see the opposite on the Friends dataset. Figure \ref{fig:main_heatmaps} shows that T5 with co-training was able to perform particularly well on question answering, but struggled to transfer to reading comprehension and personality detection. Additionally, we find that while BERT and GPT-2 are able to use character identification and personality detection as good source tasks, T5 doesn't have any consistent benefit from source tasks.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/score_deltas_by_sample_count.png}
    \caption{\textbf{Score $\Delta$ by sample count}. Sample count is on the x-axis (log scale) and score $\Delta$ is on the y-axis. Blue x's in the figure represent the average transfer $\Delta$ from a source task to all target tasks. Brown o's represent the average transfer $\Delta$ to a target task from all sources. Trend lines are a linear best-fit on the data with a 95\% confidence interval.}
    \label{fig:score_delta_by_sample_count}
\end{figure}

\paragraph{Performance Across Learning Algorithms}
Overall, we find that the co-train/fine-tune algorithm almost always performs best. In particular, we average scores for each learning algorithm across both datasets and find that the pre-train/fine-tune gets an average score of 42.85, co-train averages a score of 42.84, and co-train/fine-tune averages 44.07.
In Table \ref{tab:overall_transfer} we see that co-train/fine-tune achieves the best average score for all models and both datasets, and indeed it's average performance of 44.07 is a 2.8\% improvement over the pre-train/fine-tune and co-train algorithms. However, the aggregate score misses some nuances.

Table \ref{tab:overall_transfer} shows that co-training always improves over pre-train/fine-tune for BERT and GPT-2, but the opposite is true for T5. This is a counter-intuitive finding because this suggests that T5 isn't as good at multi-task settings or at least that it needs extra training directly on the target task. \textcolor{blue}{This adds to the idea from unicorn on rainbow, where they find the same thing for T5, but we find that this analysis depends on the model}

Looking at T5's performance on DailyDialog, we find that for top-1 scores, pre-train/fine-tune achieves the best score, but co-train/fine-tune outperforms pre-train/fine-tune on average. \textcolor{blue}{This follows the findings of RAINBOW and Ext5, but still, we show that their findings don't hold on other model architectures \cite{Lourie2021UNICORNOR}.} This finding suggests that while co-train/fine-tune does not achieve the best scores, it does act as a regularization against poor performing source tasks. We find that the bottom-1 scores for T5 on DailyDialog are 46.78, 46.69, and 48.26 for pre-train/fine-tune, co-train, and co-train/fine-tune algorithms, outperforming by over 3\%, confirming that the co-train/fine-tune algorithm does achieve the best worst-case performance. Furthermore, we find that for all datasets and models, co-train/fine-tune does get the best worst-case performance among learning algorithms. In fact, for GPT-2 on Friends the bottom-1 sources still lead to a 0.74\% improvement over the baseline.

\paragraph{Correlation By Sample Size}
One apparent feature of Figure \ref{fig:main_heatmaps} is that Dialogue Reasoning Span Extraction (DRSE) benefits greatly from task transfer. DRSE also has the fewest samples in the DailyDialog dataset, which leads to the question: How do source and target sample sizes correlate with performance? Figure \ref{fig:score_delta_by_sample_count} shows that there is not an immediately clear answer to this question. Interestingly, we find that while BERT shows no significant trend, GPT-2 and T5 display opposite trends. $\Delta$s increase for GPT-2 when target task samples increase, but $\Delta$s increase for T5 when source task samples increase. This may mean that T5 is better at learning on a low-resource target task with a more abundant source task, while GPT2 is better at boosting the performance of a target task with richer data with low-resource source task.

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/score_deltas_by_sample_ratio_for_task_type.png}
    \caption{\textbf{Score $\Delta$ by target task type}. Each line represents a different task type, defined in Table \ref{tab:dataset_info}.}
    \label{fig:task_type}
\end{figure}

By looking at the score $\Delta$ for target tasks (in brown), we observe that there is a large variance in $\Delta$, even in tasks with similar sample sizes. This variance is significantly smaller when looking at source tasks (in blue), suggesting that the number of samples from the source task actually does not have as large of an effect on $\Delta$s as the number of target task samples.

\paragraph{Correlation By Task Type}

Figure \ref{fig:task_type} demonstrates some interesting trends when comparing score $\Delta$s across different target task types. We find that span extraction is the task type which gains the most from every source task. Both span extraction and multiple choice tasks see high score improvements when their source tasks have high number of samples. This is likely due to the high-level language understanding required by both tasks, when compared with classification tasks. Also very interestingly, we find that utterance-level classification tasks, on average, see a decrease in score when transferring from source tasks with large samples. This is possibly due to language models forgetting some of the important skills learned during their large-scale pre-training, similar to the finding of \citet{pruksachatkun-etal-2020-intermediate}.

\subsection{Multi-Source Setting}

In this setting we selectively test multitask transfer on promising target tasks. For these experiments, we select the four target tasks which had the best score difference across all models and algorithms, shown in Figures \ref{fig:dd_aggregate_heatmap} and \ref{fig:friends_aggregate_heatmap} in the Appendix. We find that to be Dialogue Reasoning Span Extraction (DRSE), Dialogue-Level NLI (DNLI), Character Identification (CI), and Question Answering (QA). Given these promising target tasks, we select the three source tasks which, on average, provided the best transfer to each target, again, shown in Figures \ref{fig:dd_aggregate_heatmap} and \ref{fig:friends_aggregate_heatmap} in the Appendix. In this setting, we train models and algorithms in the same method as the single-source setting, except that when optimizing loss on a source task, we now simultaneously optimize the loss for multiple source tasks.
% To mitigate the varying sample sizes for each task, we weight the loss from a given task by it's inverse proportion of total data.

% \begin{table}[t]
%     \centering
%     \setlength{\tabcolsep}{2pt}
%     \small
%     \begin{tabular}{l l | c c | c c | c c}
%         \multicolumn{2}{r|}{\textbf{Target}} & \multicolumn{2}{c}{\textbf{DRSE}} & \multicolumn{2}{c}{\textbf{DNLI}} & \multicolumn{2}{c}{\textbf{CI}}\\
%          &  & & \multirow{2}{*}{\begin{tabular}{c}\textbf{Multi-}\\\textbf{Source}\end{tabular}} &
%           & \multirow{2}{*}{\begin{tabular}{c}\textbf{Multi-}\\\textbf{Source}\end{tabular}} &
%           & \multirow{2}{*}{\begin{tabular}{c}\textbf{Multi-}\\\textbf{Source}\end{tabular}}\\
%         & & \textbf{Top-1}& & \textbf{Top-1}& & \textbf{Top-1}& \\
%         \hline
%         \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{BERT}}}}
%         & P/F & 0.46 & -0.83 & 0.88 & 1.48 & -0.76 & -2.27\\
%         & C & 1.86 & \textbf{3.73} & 1.05 & 2.20 & \textbf{-0.27} & -1.38\\
%         & C/F & 2.58 & 3.62 & 3.55 & \textbf{4.48} & -0.48 & -0.95\\
%         \hline
%         \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{GPT-2}}}}
%         & P/F & 1.14 & 0.99 & 0.00 & -3.39 & 2.73 & 5.95 \\
%         & C & 1.59 & 2.04 & -0.81 & -0.18 & 2.70 & 1.75\\
%         & C/F & \textbf{3.43} & 3.11 & \textbf{0.46} & -0.68 & \textbf{8.81} & \textbf{8.81}\\
%         \hline
%         \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{T5}}}}
%          & P/F & -1.08 & -1.28 & 8.60 & 7.50 & \textbf{2.22} & 0.71 \\
%         & C & 2.93 & 1.00 & \textbf{8.83} & 4.11 & 0.22 & -2.13\\
%         & C/F & \textbf{3.30} & 1.88 & 5.59 & 2.96 & 1.46 & 0.40
%     \end{tabular}
%     \caption{\textbf{Multi-source score $\Delta$s from baseline.} }
%     \label{tab:targeted_setting}
% \end{table}

\begin{table}[t]
    \centering
    \small
    \begin{tabular}{l l | c | c | c | c}
        \multicolumn{2}{r|}{\textbf{Target}} & \textbf{DRSE} & \textbf{DNLI} & \textbf{CI} & \textbf{QA}\\
        \hline
        \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{BERT}}}}
        & P/F & -0.83 & +1.48& -2.27 & -0.92\\
        & C & +3.73 & +2.20 & -1.38 & +1.36\\
        & C/F & +3.62 & +4.48 & -0.95 & +3.17\\
        \hline
        \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{GPT-2}}}}
        & P/F &  +0.99 & -3.39 & +5.95 & -4.67\\
        & C & +2.04 & -0.18 & +1.75 & -3.70\\
        & C/F & +3.11 & -0.68 & +8.81 & -1.94\\
        \hline
        \parbox[t]{2mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\textbf{T5}}}}
         & P/F &  -1.28 & +7.5 & +0.71 & +0.32\\
        & C & +1.00 & +4.11 & -2.13 & +0.81\\
        & C/F & +1.88 & +2.96 & +0.40 & -0.28
    \end{tabular}
    \caption{\textbf{Multi-source score $\Delta$s from baseline.}}
    \label{tab:targeted_setting}
\end{table}

\paragraph{Multi-Source Results} Table \ref{tab:targeted_setting} shows the scores from the multi-source setting. As a comparison for these scores, we consider the average score of the top-3 sources used in the single-source setting, shown in Table \ref{tab:multisource_full} in the Appendix. We expect that the multi-source setting should generally improve performance for all models and algorithms, but find results to the contrary. Overall, We find that 6/9 multi-source algorithms outperform their average top-3 single-source counterparts in DRSE, 6/9 for DNLI, 3/9 for CI, and only 2/9 for QA. The result for DRSE is not surprising given that there is an almost unanimous benefit from source tasks, shown in Figure \ref{fig:main_heatmaps}. 

We find that 7/12 models trained with the pre-train/fine-tune algorithm outperform their average top-3 single-source counterparts, 6/12 for the co-train algorithm, and 4/12 for co-train/fine-tune. This is another unintuitive result as we found the co-train/fine-tune algorithm to perform best in the single-source setting. Interestingly, we find that GPT-2 improves in the multi-source setting on 8/12 experiments, but BERT only 5/12 and T5 in only 4/12 experiments. Finding that T5 performs the worst out of all three models is counter-intuitive as we would expect that T5, with twice as many parameters as both BERT and GPT-2, should have a higher capacity for learning multiple tasks. On the other hand, in the few-sample setting more parameters may be causing the T5 model to overfit on training data, and lose performance.

==> sections/benchmark_tracks.tex <==
\section{Benchmark Tracks}
FETA contains two tracks: \textbf{Comprehensive} and \textbf{Targeted}. 

The Comprehensive track is designed for researchers to exhaustively test their models and algorithms on task transfer by considering all pairwise combinations of tasks within a dataset. This track compares the capabilities of different models and transfer algorithms at a high level rather than on any specific task.
% Who is this track for? What does it measure?
% This track is for:
%   Researchers interested in seeing how a model/algorithm performs in a pure task transfer setting as a whole
%   More aimed at theoretical performance of a task transfer algorithm, rather than performance on any specific task
%   Researchers with resources

The Targeted track, on the other hand, contains groupings of multiple source tasks along with a target task, where the source tasks are selected based on good performance in the pairwise setting. This track allows for researchers who are more interested in a specific target task, as well as those interested in larger multi-task settings. Furthermore, the Targeted track requires only a fraction of the experiments as the Comprehensive track, encouraging participation from a wider audience.
% This track is for:
%   researchers with less resources
%   researchers interested in a specific target task
%   researchers interested in multi-task settings
%   

==> sections/introduction.tex <==
\section{Introduction}
\label{sec:intro}
% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=\columnwidth]{images/circles.png}
%     \caption{\textbf{Task Transfer Performance} on DailyDialog (top) and Friends (bottom) datasets. Computed transfer performance is demonstrated by arrows leaving from source tasks and entering target tasks. Strength of the transfer is denoted by thickness and color of edges. \ww{If you run out of space, we can show only one figure here instead of two.}}
%     \label{fig:circles}
% \end{figure}

\begin{figure}[t!]
    \centering
    \includegraphics[width=\columnwidth]{images/circles-Page-2.png}
    \caption{\textbf{Task Transfer Performance} on \feta-DailyDialog. Computed transfer performance is demonstrated by arrows leaving from source tasks and entering target tasks. Strength of the transfer is denoted by thickness and color of edges.}
    \label{fig:circles}
\end{figure}

\ww{I think the intro could be clearer. You have not emphasized enough the redundant annotation issue: for example, in NLU / dialogue understanding, one might not need separate annotations for dialogue acts, semantic parsing, emotion recognition, and relation extraction. Some of the annotations might be redundant and contain duplicate information. Task transfer and intra-dataset transfer might help. This has never been discussed.}
% Why transfer learning for dialogue?
Improving sample efficiency through transfer learning has been a long standing challenge in the machine learning and natural language processing communities \cite{transfer_91,JMLR:v6:ando05a}. Recently, transfer learning using pre-trained language models as an initial substrate has become integral to performing language tasks \cite{peters-etal-2017-semi,peters-etal-2018-deep, devlin-etal-2019-bert,radford2019language,raffel_t5}.
Dialogue data requires multiple cohesive turns with consistent speaker personalities \cite{budzianowski-etal-2018-multiwoz,urbanek-etal-2019-learning}, creating a challenge for data collection and motivating the development of techniques that improve sample efficiency in conversational AI \cite{MehriDialoGLUE2020, Shuster2020TheDD}.

% Dialogue data is generally challenging to gather and annotate\ww{The argument could be stronger, because other NLP data are difficult to gather too (e.g., multilingual data).} \cite{rashkin-etal-2019-towards, budzianowski-etal-2018-multiwoz}, motivating the development of techniques that improve sample efficiency such as transfer learning  for conversational AI \cite{MehriDialoGLUE2020, Shuster2020TheDD, simpleTOD}.

% Why task transfer in Open-domain dialogue?
Two important settings of transfer learning, namely domain adaptation and task transfer, have been studied on language tasks \cite{NEURIPS2019_4496bf24}. While domain adaptation has been studied in open-domain dialogue \cite{MehriDialoGLUE2020} and task transfer has been studied in general NLP tasks \cite{pruksachatkun-etal-2020-intermediate}, task transfer has been studied with less rigor in dialogue. Previous studies on task transfer in dialogue focus on task-oriented dialogue, have only considered 2-4 tasks, and focus on the multitask setting without a comprehensive evaluation of learning algorithms \cite{udupa-etal-2009-mint, wu-etal-2020-tod,simpleTOD}.

% What sets this work apart?
Furthermore, previous studies have focused on cross-dataset task transfer, gathering tasks annotated on disjoint datasets \cite{pruksachatkun-etal-2020-intermediate, Vu2020ExploringAP, Ye2021CrossFitAF}, but this can lead to improvements in domain adaptation being confounded as improvements in task transfer. A precise study of task transfer should be on a single data source in an intra-dataset transfer setting, as in \citet{Zamir_2018_CVPR}. However, annotating multiple tasks on a single dataset can be a challenging constraint. To the best of our knowledge, this is the first rigorous study on task transfer in dialogue and the largest intra-dataset task transfer study in NLP.

\iffalse
% What sets this work apart?
It is beneficial when studying task transfer to annotate tasks on top of a single data source in order to remove domain adaptation as a confounding variable, which can be a challenging constraint \cite{Zamir_2018_CVPR}.
% In comparison with prior studies on task transfer in NLP which do not account for domain adaptation \cite{pruksachatkun-etal-2020-intermediate, Vu2020ExploringAP, Ye2021CrossFitAF}, in this work we aim to measure task transfer accurately. \textcolor{blue}{seems a bit harsh. Does somebody have an idea for nicer phrasing?}
To the best of our knowledge, this is the first rigorous study on task transfer in open-domain dialogue.
\fi

% This paper introduces FETA
In this work, we create \feta, a benchmark for few-sample task transfer for language understanding in open-domain dialogue with 17 total tasks. \feta\;datasets cover a variety of properties (dyadic vs. multi-party, anonymized vs. recurring speaker, varying dialogue lengths) and task types (utterance-level classification, dialogue-level classification, span extraction, multiple choice) as well as supporting a wide variety of data quantities.

% How do we study FETA, and what is a high-level result of the study
We study task transfer on \feta\; by comparing three task transfer algorithms on three commonly used language models. In this work, we consider both the single-source and multi-source settings of task transfer. Figure \ref{fig:circles} illustrates some results in the single-source setting. For example, we find that Dialogue Reasoning Span Extraction
% and Character Identification benefit
benefits
from nearly all source tasks. On the other hand, Adversarial Response Selection and Emotion Recognition provide benefits to many target tasks when utilized as a source task.

In this study, we find that: (i) Span extraction tasks gain the most as a target, especially with few samples. (ii) Scores averaged across all source tasks significantly underperform compared with the best source task, motivating further research into determining optimal source tasks. (iii) All trends are dependent on the model. (iv) Multi-source training gets mixed improvements over single-source, again motivating a better understanding of the complex relationship between source and target tasks.

\feta\;provides a resource for a variety of future studies, e.g. on the generalizability of model architectures, and pre-training datasets that enable efficient transfer. In addition to task transfer, \feta\;can also facilitate the study of continual and multitask learning.

In summary, our main contributions are:
\begin{itemize}
    \item We create the first large-scale benchmark for task transfer in open-domain dialogue, with 132 source-target task pairs.
    \item Extensive experimentation on \feta\;in both the single-source and multi-source settings, as well as an analysis comparing models, learning algorithms, sample sizes, and task types.
    \item A readily extensible transfer learning framework allowing for rapid experimentation and an online leaderboard encouraging deeper research into task transfer.
\end{itemize}
